Resource Allocation in Disaggregated Data Centre Systems with Reinforcement Learning

Resource-disaggregated data centres (RDDC) propose a resource-centric, and high-utilisation architecture for data centres (DC), avoiding resource fragmentation and enabling arbitrarily sized resource pools to be allocated to tasks, rather than server-sized ones. RDDCs typically impose greater demand on the network, requiring more infrastructure and increasing cost and power, so new resource allocation algorithms that co-manage both server and networks resources are essential to ensure that allocation is not bottlenecked by the network, and that requests can be served successfully with minimal networking resources. We apply reinforcement learning (RL) to this problem for the first time and show that an RL policy based on graph neural networks can learn resource allocation policies end-to-end that outperform previous hand-engineered heuristics by up to 22.0\%, 42.6\% and 22.6\% for acceptance ratio, CPU and memory utilisation respectively, maintain performance when scaled up to RDDC topologies with $10^2\times$ more nodes than those seen during training and can achieve comparable performance to the best baselines while using $5.3\times$ less network resources.

==> submission/notes.tex <==
\section{Notes}
\subsection{Introduction/Literature Review}

\subsection{Results collection revision}

\subsubsection{Channels per link (per tier)}
\subsubsection*{14/09/21}

Run grid search baseline rollout over following variations of channels per link at each tier of link:

\begin{itemize}
    \item \textbf{SRLink:} [8,16,32]
    \item \textbf{RALink:} [8,16,32]
    \item \textbf{ACLink:} [8,16,32]
\end{itemize}

with a revised alpha-topology that has 16 servers per rack and 16 CPU and memory units per server.

Currently only testing on uniform requests (which still request up to half of an empty racks worth of resources.

Have also hardcoded the network request to always be 1, so that the feature normalisation procedure implemented in the environment is correct.

